Teaching LLMs to Plan: Logical Chain-of-Thought Instruction Tuning for Symbolic Planning

Large language models (LLMs) have demonstrated impressive capabilities across diverse tasks, yet their ability to perform structured symbolic planning remains limited, particularly in domains requiring formal representations like the Planning Domain Definition Language (PDDL). In this paper, we present a novel instruction tuning framework, PDDL-Instruct, designed to enhance LLMs' symbolic planning capabilities through logical chain-of-thought reasoning. Our approach focuses on teaching models to rigorously reason about action applicability, state transitions, and plan validity using explicit logical inference steps. By developing instruction prompts that guide models through the precise logical reasoning required to determine when actions can be applied in a given state, we enable LLMs to self-correct their planning processes through structured reflection. The framework systematically builds verification skills by decomposing the planning process into explicit reasoning chains about precondition satisfaction, effect application, and invariant preservation. Experimental results on multiple planning domains show that our chain-of-thought reasoning based instruction-tuned models are significantly better at planning, achieving planning accuracy of up to 94% on standard benchmarks, representing a 66% absolute improvement over baseline models. This work bridges the gap between the general reasoning capabilities of LLMs and the logical precision required for automated planning, offering a promising direction for developing better AI planning systems.

==> prompts/cot_feedback_correct_binary.tex <==
Phase 2 CoT with Binary Feedback Prompt

[INSTRUCTION] You previously generated a plan with step-by-step reasoning. The 
validator has provided feedback on your reasoning. Use this feedback to 
generate a corrected plan with improved logical reasoning.

[DOMAIN]
(define (domain blocksworld)
  (:requirements :strips)
  (:predicates 
    (on ?x ?y) (ontable ?x) (clear ?x) (handempty) (holding ?x))
  (:action pick-up
    :parameters (?x)
    :precondition (and (clear ?x) (ontable ?x) (handempty))
    :effect (and (not (ontable ?x)) (not (handempty)) 
                 (not (clear ?x)) (holding ?x)))
  (:action put-down
    :parameters (?x)
    :precondition (holding ?x)
    :effect (and (not (holding ?x)) (handempty) 
                 (ontable ?x) (clear ?x)))
  (:action stack
    :parameters (?x ?y)
    :precondition (and (holding ?x) (clear ?y))
    :effect (and (not (holding ?x)) (not (clear ?y)) 
                 (handempty) (on ?x ?y) (clear ?x)))
  (:action unstack
    :parameters (?x ?y)
    :precondition (and (on ?x ?y) (clear ?x) (handempty))
    :effect (and (not (on ?x ?y)) (not (handempty)) 
                 (holding ?x) (clear ?y))))

[PROBLEM]
(define (problem bw-simple)
  (:domain blocksworld)
  (:objects a b c)
  (:init (ontable a) (ontable b) (ontable c) 
         (clear a) (clear b) (clear c) (handempty))
  (:goal (and (on a b) (on b c))))

[PREVIOUS PLAN]
Step 1: (pick-up b) - VALID
Step 2: (stack b c) - VALID  
Step 3: (pick-up a) - VALID
Step 4: (stack a b) - VALID

[VAL FEEDBACK]
Plan Validation details
-----------------------
Checking next happening (time 1)
Deleting (ontable b)
Deleting (handempty)
Deleting (clear b)
Adding (holding b)

Checking next happening (time 2)
Deleting (holding b)
Deleting (clear c)
Adding (handempty)
Adding (on b c)
Adding (clear b)

Checking next happening (time 3)
Deleting (ontable a)
Deleting (handempty)
Deleting (clear a)
Adding (holding a)

Checking next happening (time 4)
Deleting (holding a)
Deleting (clear b)
Adding (handempty)
Adding (on a b)
Adding (clear a)
Plan executed successfully - checking goal
Plan valid


==> prompts/cot_feedback_correct_detailed.tex <==
Phase 2 CoT with Binary Feedback Prompt

[INSTRUCTION] You previously generated a plan with step-by-step reasoning. The 
validator has provided feedback on your reasoning. Use this feedback to 
generate a corrected plan with improved logical reasoning.

[DOMAIN]
(define (domain blocksworld)
  (:requirements :strips)
  (:predicates 
    (on ?x ?y) (ontable ?x) (clear ?x) (handempty) (holding ?x))
  (:action pick-up
    :parameters (?x)
    :precondition (and (clear ?x) (ontable ?x) (handempty))
    :effect (and (not (ontable ?x)) (not (handempty)) 
                 (not (clear ?x)) (holding ?x)))
  (:action put-down
    :parameters (?x)
    :precondition (holding ?x)
    :effect (and (not (holding ?x)) (handempty) 
                 (ontable ?x) (clear ?x)))
  (:action stack
    :parameters (?x ?y)
    :precondition (and (holding ?x) (clear ?y))
    :effect (and (not (holding ?x)) (not (clear ?y)) 
                 (handempty) (on ?x ?y) (clear ?x)))
  (:action unstack
    :parameters (?x ?y)
    :precondition (and (on ?x ?y) (clear ?x) (handempty))
    :effect (and (not (on ?x ?y)) (not (handempty)) 
                 (holding ?x) (clear ?y))))

[PROBLEM]
(define (problem bw-simple)
  (:domain blocksworld)
  (:objects a b c)
  (:init (ontable a) (ontable b) (ontable c) 
         (clear a) (clear b) (clear c) (handempty))
  (:goal (and (on a b) (on b c))))

[PREVIOUS PLAN]
Step 1: (pick-up b) - VALID
Step 2: (stack b c) - VALID  
Step 3: (pick-up a) - VALID
Step 4: (stack a b) - VALID

[VAL FEEDBACK]
Plan Validation details
-----------------------
Checking next happening (time 1)
Deleting (ontable b)
Deleting (handempty)
Deleting (clear b)
Adding (holding b)

Checking next happening (time 2)
Deleting (holding b)
Deleting (clear c)
Adding (handempty)
Adding (on b c)
Adding (clear b)

Checking next happening (time 3)
Deleting (ontable a)
Deleting (handempty)
Deleting (clear a)
Adding (holding a)

Checking next happening (time 4)
Deleting (holding a)
Deleting (clear b)
Adding (handempty)
Adding (on a b)
Adding (clear a)
Plan executed successfully - checking goal
Plan valid

[EXPLANATION] This plan is VALID. Here is the analysis of each action:

[Action 1: (pick-up b)]
- Preconditions: (clear b), (ontable b), (handempty)
- Initial state satisfies all preconditions: b is clear, b is on table, and hand is empty
- Effects: b is now held, hand is not empty, b is not on table, b is not clear
- Resulting state: (ontable a) (ontable c) (clear a) (clear c) (holding b)

[Action 2: (stack b c)]
- Preconditions: (holding b), (clear c)  
- Current state satisfies preconditions: holding b and c is clear
- Effects: b is stacked on c, hand becomes empty, c is no longer clear, b becomes clear
- Resulting state: (ontable c) (ontable a) (clear a) (clear b) (on b c) (handempty)

[Action 3: (pick-up a)]
- Preconditions: (clear a), (ontable a), (handempty)
- Initial state satisfies all preconditions: a is clear, a is on table, and hand is empty
- Effects: a is now held, hand is not empty, a is not on table, a is not clear
- Resulting state: (on b c) (ontable c) (clear b) (holding a)

[Action 4: (stack a b)]
- Preconditions: (holding a), (clear b)  
- Current state satisfies preconditions: holding a and b is clear
- Effects: a is stacked on b, hand becomes empty, b is no longer clear, a becomes clear
- Resulting state: (ontable c) (on b c) (on a b) (clear a) (handempty)

The plan succeeds.




==> prompts/cot_feedback_incorrect_binary.tex <==
Phase 2 CoT with Binary Feedback Prompt

[INSTRUCTION] You previously generated a plan with step-by-step reasoning. The 
validator has provided feedback on your reasoning. Use this feedback to 
generate a corrected plan with improved logical reasoning.

[DOMAIN]
(define (domain blocksworld)
  (:requirements :strips)
  (:predicates 
    (on ?x ?y) (ontable ?x) (clear ?x) (handempty) (holding ?x))
  (:action pick-up
    :parameters (?x)
    :precondition (and (clear ?x) (ontable ?x) (handempty))
    :effect (and (not (ontable ?x)) (not (handempty)) 
                 (not (clear ?x)) (holding ?x)))
  (:action put-down
    :parameters (?x)
    :precondition (holding ?x)
    :effect (and (not (holding ?x)) (handempty) 
                 (ontable ?x) (clear ?x)))
  (:action stack
    :parameters (?x ?y)
    :precondition (and (holding ?x) (clear ?y))
    :effect (and (not (holding ?x)) (not (clear ?y)) 
                 (handempty) (on ?x ?y) (clear ?x)))
  (:action unstack
    :parameters (?x ?y)
    :precondition (and (on ?x ?y) (clear ?x) (handempty))
    :effect (and (not (on ?x ?y)) (not (handempty)) 
                 (holding ?x) (clear ?y))))

[PROBLEM]
(define (problem bw-simple)
  (:domain blocksworld)
  (:objects a b c)
  (:init (ontable a) (ontable b) (ontable c) 
         (clear a) (clear b) (clear c) (handempty))
  (:goal (and (on a b) (on b c))))

[PREVIOUS PLAN]
Step 1: (pick-up b) - VALID
Step 2: (stack b c) - VALID  
Step 3: (stack a b) - INVALID

[VAL FEEDBACK]
Plan Validation details
-----------------------
Checking next happening (time 1)
Deleting (ontable b)
Deleting (handempty)
Deleting (clear b)
Adding (holding b)

Checking next happening (time 2)
Deleting (holding b)
Deleting (clear c)
Adding (handempty)
Adding (on b c)
Adding (clear b)

Checking next happening (time 3)
Plan failed because of unsatisfied precondition in:
(stack a b)

Plan failed to execute

[GENERATE CORRECTED PLAN WITH REASONING]


==> prompts/cot_feedback_incorrect_detailed.tex <==
Phase 2 CoT with Binary Feedback Prompt

[INSTRUCTION] You previously generated a plan with step-by-step reasoning. The 
validator has provided feedback on your reasoning. Use this feedback to 
generate a corrected plan with improved logical reasoning.

[DOMAIN]
(define (domain blocksworld)
  (:requirements :strips)
  (:predicates 
    (on ?x ?y) (ontable ?x) (clear ?x) (handempty) (holding ?x))
  (:action pick-up
    :parameters (?x)
    :precondition (and (clear ?x) (ontable ?x) (handempty))
    :effect (and (not (ontable ?x)) (not (handempty)) 
                 (not (clear ?x)) (holding ?x)))
  (:action put-down
    :parameters (?x)
    :precondition (holding ?x)
    :effect (and (not (holding ?x)) (handempty) 
                 (ontable ?x) (clear ?x)))
  (:action stack
    :parameters (?x ?y)
    :precondition (and (holding ?x) (clear ?y))
    :effect (and (not (holding ?x)) (not (clear ?y)) 
                 (handempty) (on ?x ?y) (clear ?x)))
  (:action unstack
    :parameters (?x ?y)
    :precondition (and (on ?x ?y) (clear ?x) (handempty))
    :effect (and (not (on ?x ?y)) (not (handempty)) 
                 (holding ?x) (clear ?y))))

[PROBLEM]
(define (problem bw-simple)
  (:domain blocksworld)
  (:objects a b c)
  (:init (ontable a) (ontable b) (ontable c) 
         (clear a) (clear b) (clear c) (handempty))
  (:goal (and (on a b) (on b c))))

[PREVIOUS PLAN]
Step 1: (pick-up b) - VALID
Step 2: (stack b c) - VALID  
Step 3: (stack a b) - INVALID

[VAL FEEDBACK]
Plan Validation details
-----------------------
Checking next happening (time 1)
Deleting (ontable b)
Deleting (handempty)
Deleting (clear b)
Adding (holding b)

Checking next happening (time 2)
Deleting (holding b)
Deleting (clear c)
Adding (handempty)
Adding (on b c)
Adding (clear b)

Checking next happening (time 3)
Plan failed because of unsatisfied precondition in:
(stack a b)

Plan failed to execute

Plan Repair Advice:

(stack a b) has an unsatisfied precondition at time 3
(Set (holding a) to true)

[EXPLANATION] This plan is INVALID. Here is the analysis of each action:

[Action 1: (pick-up b)]
- Preconditions: (clear b), (ontable b), (handempty)
- Initial state satisfies all preconditions: b is clear, b is on table, and hand is empty
- Effects: b is now held, hand is not empty, b is not on table, b is not clear
- Resulting state: (ontable a) (ontable c) (clear a) (clear c) (holding b)

[Action 2: (stack b c)]
- Preconditions: (holding b), (clear c)  
- Current state satisfies preconditions: holding b and c is clear
- Effects: b is stacked on c, hand becomes empty, c is no longer clear, b becomes clear
- Resulting state: (ontable c) (ontable a) (clear a) (clear b) (on b c) (handempty)

[Action 3: (stack a b)]
- Preconditions: (holding a), (clear b)
- Current state: (ontable c) (ontable a) (clear a) (clear b) (on b c) (handempty)
- VIOLATION: The precondition (holding a) is not satisfied - the hand is empty and a is on the table

[GENERATE CORRECTED PLAN WITH REASONING]


==> prompts/cot_generation.tex <==
[INSTRUCTION] Generate a plan for the given problem using step-by-step reasoning. For each action, explicitly verify preconditions, apply effects, and track state changes.

[DOMAIN]
(define (domain blocksworld)
  (:requirements :strips)
  (:predicates 
    (on ?x ?y) (ontable ?x) (clear ?x) (handempty) (holding ?x))
  (:action pick-up
    :parameters (?x)
    :precondition (and (clear ?x) (ontable ?x) (handempty))
    :effect (and (not (ontable ?x)) (not (handempty)) 
                 (not (clear ?x)) (holding ?x)))
  (:action put-down
    :parameters (?x)
    :precondition (holding ?x)
    :effect (and (not (holding ?x)) (handempty) 
                 (ontable ?x) (clear ?x)))
  (:action stack
    :parameters (?x ?y)
    :precondition (and (holding ?x) (clear ?y))
    :effect (and (not (holding ?x)) (not (clear ?y)) 
                 (handempty) (on ?x ?y) (clear ?x)))
  (:action unstack
    :parameters (?x ?y)
    :precondition (and (on ?x ?y) (clear ?x) (handempty))
    :effect (and (not (on ?x ?y)) (not (handempty)) 
                 (holding ?x) (clear ?y))))

[PROBLEM]
(define (problem bw-tower)
  (:domain blocksworld)  
  (:objects a b c)
  (:init (on c b) (ontable b) (ontable a) 
         (clear c) (clear a) (handempty))
  (:goal (and (on a c) (on c b))))

[EXPECTED RESPONSE]

Initial State Analysis:
Current state: (on c b), (ontable b), (ontable a), (clear c), (clear a), (handempty)
Goal: (on a c), (on c b)

[STEP BY STEP PLANNING]

[Step 1: State s0 → Action a1 → State s1]
- Current state s0: (on c b), (ontable b), (ontable a), (clear c), (clear a), (handempty)
- Proposed action a1: (pick-up a)
- Precondition check:
  - (clear a): TRUE in s0
  - (ontable a): TRUE in s0  
  - (handempty): TRUE in s0
- Action is APPLICABLE
- Effect application:
  - Add: (holding a)
  - Delete: (ontable a), (handempty), (clear a)
- Resulting state s1: (on c b), (ontable b), (clear c), (holding a)

[Step 2: State s1 → Action a2 → State s2]
- Current state s1: (on c b), (ontable b), (clear c), (holding a)
- Proposed action a2: (stack a c)
- Precondition check:
  - (holding a): TRUE in s1
  - (clear c): TRUE in s1
- Action is APPLICABLE
- Effect application:
  - Add: (on a c), (handempty), (clear a)
  - Delete: (holding a), (clear c)
- Resulting state s2: (on c b), (ontable b), (on a c), (handempty), (clear a)

[GOAL ACHIEVEMENT CHECK]
Required: (on a c), (on c b)
Current state s2: (on c b), (ontable b), (on a c), (handempty), (clear a)
- (on a c): TRUE in s2
- (on c b): TRUE in s2 
Goal is ACHIEVED.

[FINAL PLAN] (pick-up a), (stack a c)

==> prompts/incorrect_initial.tex <==
[INSTRUCTION] Given the following PDDL domain and problem, analyze the provided plan and explain why each action is valid.

[DOMAIN]
(define (domain blocksworld)
  (:requirements :strips)
  (:predicates 
    (on ?x ?y) (ontable ?x) (clear ?x) (handempty) (holding ?x))
  (:action pick-up
    :parameters (?x)
    :precondition (and (clear ?x) (ontable ?x) (handempty))
    :effect (and (not (ontable ?x)) (not (handempty)) 
                 (not (clear ?x)) (holding ?x)))
  (:action put-down
    :parameters (?x)
    :precondition (holding ?x)
    :effect (and (not (holding ?x)) (handempty) 
                 (ontable ?x) (clear ?x)))
  (:action stack
    :parameters (?x ?y)
    :precondition (and (holding ?x) (clear ?y))
    :effect (and (not (holding ?x)) (not (clear ?y)) 
                 (handempty) (on ?x ?y) (clear ?x)))
  (:action unstack
    :parameters (?x ?y)
    :precondition (and (on ?x ?y) (clear ?x) (handempty))
    :effect (and (not (on ?x ?y)) (not (handempty)) 
                 (holding ?x) (clear ?y))))

[PROBLEM]
(define (problem bw-simple)
  (:domain blocksworld)
  (:objects a b c)
  (:init (ontable a) (ontable b) (ontable c) 
         (clear a) (clear b) (clear c) (handempty))
  (:goal (and (on a b) (on b c))))

[PLAN]
1. (stack a b)
2. (stack b c)

[EXPECTED RESPONSE] This plan is INVALID. Let me analyze each action:

[Action 1: (stack a b)]
- Preconditions: (holding a), (clear b)
- Current state: (ontable a) (ontable b) (ontable c) (clear a) (clear b) (clear c) (handempty)
- VIOLATION: The precondition (holding a) is not satisfied - the hand is empty and a is on the table
- To stack a on b, we must first pick up a

[Action 2: (stack b c)]
- Since Action 1 failed, this action cannot be evaluated in a valid state sequence
- Even if Action 1 succeeded, we would need to be holding b to stack it on c

The plan fails because it attempts to stack blocks without first picking them up. The correct sequence would be: (pick-up a), (stack a b), (pick-up b), (stack b c).

==> prompts/initial.tex <==
[INSTRUCTION] Given the following PDDL domain and problem, analyze the provided plan and explain why each action is valid.

[DOMAIN]
(define (domain blocksworld)
  (:requirements :strips)
  (:predicates 
    (on ?x ?y) (ontable ?x) (clear ?x) (handempty) (holding ?x))
  (:action pick-up
    :parameters (?x)
    :precondition (and (clear ?x) (ontable ?x) (handempty))
    :effect (and (not (ontable ?x)) (not (handempty)) 
                 (not (clear ?x)) (holding ?x)))
  (:action put-down
    :parameters (?x)
    :precondition (holding ?x)
    :effect (and (not (holding ?x)) (handempty) 
                 (ontable ?x) (clear ?x)))
  (:action stack
    :parameters (?x ?y)
    :precondition (and (holding ?x) (clear ?y))
    :effect (and (not (holding ?x)) (not (clear ?y)) 
                 (handempty) (on ?x ?y) (clear ?x)))
  (:action unstack
    :parameters (?x ?y)
    :precondition (and (on ?x ?y) (clear ?x) (handempty))
    :effect (and (not (on ?x ?y)) (not (handempty)) 
                 (holding ?x) (clear ?y))))

[PROBLEM]
(define (problem bw-simple)
  (:domain blocksworld)
  (:objects a b c)
  (:init (ontable a) (ontable b) (ontable c) 
         (clear a) (clear b) (clear c) (handempty))
  (:goal (and (on a b) (on b c))))


[PLAN]
1. (pick-up b)
2. (stack b c)
3. (pick-up a)  
4. (stack a b)

[EXPECTED RESPONSE] This plan is VALID. Let me analyze each action:

[Action 1: (pick-up b)]
- Preconditions: (clear b), (ontable b), (handempty)
- Initial state satisfies all preconditions: b is clear, b is on table, and hand is empty
- Effects: b is now held, hand is not empty, b is not on table, b is not clear
- Resulting state: (ontable a) (ontable c) (clear a) (clear c) (holding b)

[Action 2: (stack b c)]
- Preconditions: (holding b), (clear c)  
- Current state satisfies preconditions: holding b and c is clear
- Effects: b is stacked on c, hand becomes empty, c is no longer clear, b becomes clear
- Resulting state: (ontable c) (ontable a) (clear a) (clear b) (on b c) (handempty)

[Action 3: (pick-up a)]
- Preconditions: (clear a), (ontable a), (handempty)
- Initial state satisfies all preconditions: a is clear, a is on table, and hand is empty
- Effects: a is now held, hand is not empty, a is not on table, a is not clear
- Resulting state: (on b c) (ontable c) (clear b) (holding a)

[Action 4: (stack a b)]
- Preconditions: (holding a), (clear b)  
- Current state satisfies preconditions: holding a and b is clear
- Effects: a is stacked on b, hand becomes empty, b is no longer clear, a becomes clear
- Resulting state: (ontable c) (on b c) (on a b) (clear a) (handempty)

The plan succeeds because a is stacked on b, and b is stacked on c.
